A Cyberinfrastructure for BigData Transportation Engineering

Big Data-driven transportation engineering has the potential to improve utilization of road infrastructure, decrease traffic fatalities, improve fuel consumption, decrease construction worker injuries, among others. Despite these benefits, research on Big Data-driven transportation engineering is difficult today due to the computational expertise required to get started. This work proposes BoaT, a transportation-specific programming language, and it's Big Data infrastructure that is aimed at decreasing this barrier to entry. Our evaluation that uses over two dozen research questions from six categories show that research is easier to realize as a BoaT computer program, an order of magnitude faster when this program is run, and exhibits 12-14x decrease in storage requirements.

==> examples/motiv.tex <==

\newcommand*{\vcenteredhbox}[1]{\begingroup
	\setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}

\begin{figure}[ht]
	\begin{center}
		\begin{minipage}[t]{\textwidth}
			\begin{center}
				\textbf{Java}
			\end{center}
			\vspace{-1em}
			\input{examples/motivjava}
		\end{minipage}
		\begin{minipage}[t]{0.55\textwidth}
			\begin{center}
				\textbf{\lang}
			\end{center}
			\vspace{-1em}
			\input{examples/motivboa}
		
			
			\begin{center}
				\textbf{{\em Performance Results}}\\
				\vspace{0.5em}
				% \begin{scriptsize}
				% \rowcolors{2}{white}{gray!25}
				% \begin{tabular}{|c|c|c|c|}
				% \hline
				% \textbf{Input Size} & \multicolumn{3}{c|}{\textbf{Execution Time}}\\
				% \cline{2-4}
				% \textbf{(projects)} & \textbf{Java} & \textbf{\lang} & \textbf{Speedup}\\
				% \hline
				% 6k   &  2m:26s & 30s & 4.9x\\
				% \hline
				% 60k  & 37m:57s & 33s & 69x\\
				% \hline
				% 620k & 5h:31m & 3m:08s & 105.6x\\
				% \hline
				% \end{tabular}
				% \end{scriptsize}
				 \includegraphics[width=0.95\linewidth]{DataReduction}
			\end{center}
		\end{minipage}
		\caption{Programs for answering ``What are the churn rates for all
			Java projects that use SVN?'' and performance results on three input
			sizes.}
		\label{fig:motivating-example}
	\end{center}
\end{figure}

==> grammar.tex <==
%{grammar}, needs {obey}

%\newcommand{\heading}[1]{\vspace{3ex}{\noindent#1}\vspace{1.5ex}}
\newcommand{\goesto}{\mbox{$::=$}}
\newcommand{\arbno}[1]{#1\hbox{\rm*}}
\newcommand{\nonterm}[1]{\mbox{$\langle$#1$\rangle$}}

\newenvironment{grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{mathGrammar}{
  \def\:{\goesto{}}
  \def\|{\hbox{$\vert$}}
   \begin{displaymath}%
     \tt \obeyspaces%
}%
{\unskip\end{displaymath}}

% Commented grammars

% length before comments start on right
\newlength{\BEFOREGRAMCOMMENTLEN}
\setlength{\BEFOREGRAMCOMMENTLEN}{7cm}

% style of text inside quotations
\newcommand{\GRAMCOMMENTSTYLE}[1]{\texttt{#1}}

\newenvironment{commented-grammar}{%
\begin{grammar}%
\qquad \= $\vert$ \= \qquad \hspace*{\BEFOREGRAMCOMMENTLEN} \= \kill%
}{\end{grammar}}%

\newcommand{\gramcomment}[1]{\textrm{``\GRAMCOMMENTSTYLE{#1}''}}

% Compressed tabular grammar - takes less space
%
\newenvironment{cgrammar}{
\def\|{$\vert$}
\begin{tabular}{>{\raggedright}p{1.5cm}>{\raggedright}p{0.8cm}>{\raggedright}p{5.5cm}}%
}{\end{tabular}}%
% Production takes three parameters
% name, start symbol, production
% TODO: Extend using ithen package so that it is only defined within the cgrammar
% package.
\newcommand{\production}[3]{\mbox{#1} & \nonterm{#2}~\goesto & #3 \tabularnewline}


==> macros.tex <==
\usepackage{relsize}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{url}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{rotating}
\usepackage{colortbl}
\usepackage{tabularx}
\usepackage[table]{xcolor}
\usepackage{xspace}

\usepackage{epsfig}
\usepackage{subfigure}
\usepackage{multirow}
\graphicspath{{figures/}}
\usepackage{graphicx}

\input{tex-helpers/obey}
\input{tex-helpers/grammar}
\renewcommand{\nonterm}[1]{\mbox{\textit{#1}}}
\newcommand{\oneormore}[1]{#1\ensuremath{^+}}

\usepackage{listings}

\usepackage{algorithm}
\usepackage{algorithmic}


\tolerance=50000


\definecolor{lightgray}{gray}{0.97}
\definecolor{codeblue}{rgb}{0.13,0.13,1}
\definecolor{OliveGreen}{cmyk}{0.64,0,0.95,0.40}
\definecolor{DarkGreen}{cmyk}{0.40,0,0.50,0.15}
\definecolor{purple}{cmyk}{0.41,0.73,0,0}
\definecolor{LightRed}{cmyk}{0,0.682,0.728,0}

\makeatletter
\lst@Key{countblanklines}{true}[t]%
{\lstKV@SetIf{#1}\lst@ifcountblanklines}

\lst@AddToHook{OnEmptyLine}{%
	\lst@ifnumberblanklines\else%
	\lst@ifcountblanklines\else%
	\advance\c@lstnumber-\@ne\relax%
	\fi%
	\fi}
\makeatother

\lstset{
	language=bash,
	mathescape=false, escapechar=@,
	backgroundcolor=\color{lightgray},
	basicstyle=\relsize{-1}\ttfamily,
	keywordstyle=\color{codeblue},
	emphstyle=\color{purple},
	emphstyle={[2]\color{LightRed}},
	commentstyle=\color{DarkGreen},
	stringstyle=\color{OliveGreen},
	numberstyle=\tiny,
	numbers=left, stepnumber=1,
	numberblanklines=false,
	numbersep=-1em,
	frame=none, framexleftmargin=0pt, framexrightmargin=0pt, 
	columns=fullflexible, breaklines=true,
	keepspaces=true, showspaces=false, showstringspaces=false,
	showtabs=false, tabsize=2,
	morestring=[b]`,
	morekeywords={input,exists,foreach,ifall,output,of,weight,stop,visit,before,after},
	emph={int,string,bool,time,array,stack,map,visitor,%
		true,false,%
		top,sum,mean,maximum,minimum,set,collection,%
		County, Grid },
	emph={[2]getspeed,%
		format,def,len,match,lowercase,yearof,haskey,remove,strfind,push,pop},
}


\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}

\newcommand{\etal}{~\textit{et al.}\@\xspace}
\newcommand{\lang}{\textit{Boa}\xspace}

\renewcommand\floatpagefraction{.99}
\renewcommand\topfraction{.99}
\renewcommand\bottomfraction{.90}
\renewcommand\textfraction{.01}

\clubpenalty = 10000
\widowpenalty = 10000
\displaywidowpenalty = 10000

==> macros2.tex <==
% $Id: macros.tex,v 1.2 2012/04/18 05:59:45 hridesh Exp $
\usepackage[pdftex]{hyperref}
\frenchspacing
\usepackage{mathptmx}

%\usepackage{cite}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{url}
%\usepackage{cite}
\usepackage{amsmath}
% \usepackage{fancyhdr}
%\usepackage{fancyvrb}
%\usepackage{fancybox}
\usepackage{color}
\usepackage{colortbl}
\usepackage{mathpartir}
\usepackage{amssymb}
\usepackage{xspace}
\usepackage{comment}
\usepackage{graphicx}
\graphicspath{{figures/}}
%\usepackage{epsfig}
%\usepackage{wrapfig}
\usepackage{multirow}
%\usepackage{subfig}

% Added listing for code listings
\usepackage{listings}
\usepackage{relsize}
%\usepackage{stfloats}
\usepackage{fixltx2e}

% formatting for grammars
\input{obey}
\input{grammar}

%\newcommand{\panini}{P\={a}\={n}ini\xspace}
%\newcommand{\panini}{\textsf{java}$_c$\xspace}
\newcommand{\panini}{\textsl{OpenEffectJ}\xspace}

% Type checking macros
% change symbol type of : from mathrel 
%\DeclareMathSymbol{:}{\mathbin}{operators}{"3A} 
\newcommand{\OK}{\mbox{OK}}
\newcommand{\OKin}{\mbox{OK in }}
\newcommand{\inC}{\mbox{in }c}
\newcommand{\isType}{\mbox{\textit{isType}}}
\newcommand{\validFields}{\mbox{\textit{validF}}}
\newcommand{\isClass}{\mbox{\textit{isClass}}}
\newcommand{\isHandler}{\mbox{\textit{isHandler}}}
\newcommand{\Types}{\mbox{\textit{Types}}}
\newcommand{\Names}{\mbox{\textit{Names}}}
\newcommand{\TypeEnv}{\mbox{\textit{TypeEnv}}}
\newcommand*{\findMeth}{\auxFunc{findMeth}}
\newcommand*{\fieldsOf}{\auxFunc{fields}}
\newcommand*{\fieldName}{\auxFunc{fieldName}}
\newcommand*{\checkMethods}{\auxFunc{methE}}
\newcommand*{\methodEffect}{\auxFunc{me}}
\newcommand*{\typeOfField}{\auxFunc{typeOfF}}
\newcommand*{\typeOf}{\auxFunc{typeOf}}
\newcommand*{\dom}{\auxFunc{dom}}
\newcommand*{\rng}{\auxFunc{rng}}
\newcommand*{\isAnn}{\auxFunc{annotated}}
\newcommand*{\updateEffect}{\auxFunc{update}}
\newcommand*{\reversePointer}{\auxFunc{reverse}}
\newcommand*{\reversePoint}{\auxFunc{reverseP}}
\newcommand*{\fixPoint}{\auxFunc{fixPoint}}
\newcommand*{\updateOther}{\auxFunc{updateOther}}
\newcommand*{\updateMethodEffect}{\auxFunc{updateEff}}
\newcommand*{\updateSingleMethodEffect}{\auxFunc{updateMeth}}
\newcommand*{\updateSingleEffect}{\auxFunc{concretize}}
\newcommand*{\updateForkEffect}{\auxFunc{updateFork}}
\newcommand*{\updateQueue}{\auxFunc{updateQ}}
\newcommand*{\getActive}{\auxFunc{active}\xspace}
\newcommand*{\field}{\auxFunc{field}}
\newcommand{\fdecl}{\mbox{\textit{fdecl}}}
\newcommand*{\fieldOf}{\auxFunc{fieldOf}}
\newcommand*{\getOpen}{\auxFunc{getOpen}}
\newcommand{\NPE}{\mbox{\textit{NPE}}}

% Reserved words (in math mode)
\newcommand{\Extends}{\mbox{\texttt{\textbf{extends}}}}
\newcommand{\Implements}{\mbox{\texttt{\textbf{implements}}}}
\newcommand{\This}{\mbox{\texttt{\textbf{this}}}}
\newcommand{\EV}{\mbox{\texttt{\textbf{event}}~}}
\newcommand{\Cast}{\mbox{\texttt{\textbf{cast}}}}
\newcommand{\New}{\mbox{\texttt{\textbf{new}}~}}
\newcommand{\Null}{\mbox{\texttt{\textbf{null}}}}
\newcommand{\Chain}{\mbox{\texttt{\textbf{chain}}~}}
\newcommand{\Under}{\mbox{\texttt{\textbf{under}}~}}
\newcommand{\If}{\mbox{\texttt{\textbf{if}}}}
\newcommand{\Then}{\mbox{\texttt{\textbf{then}}}}
\newcommand{\Else}{\mbox{\texttt{\textbf{else}}}}
\newcommand{\While}{\mbox{\texttt{\textbf{while}}}}

% Aux functions
\newcommand{\auxFunc}[1]{\ensuremath{\mathop{\mathit{#1}}}}
\newcommand*{\override}{\auxFunc{override}}

% types
\newcommand{\POWERSET}[1]{\mbox{\textit{PowerSet}}(#1)}
\newcommand{\delete}{\mbox{\textit{delete}}}
\newcommand{\mklist}{\mbox{\textit{mksupers}}}
\newcommand{\uminus}{\mbox{$\cup\!\!\!\!-$}}
\newcommand{\iminus}{\mbox{$\cap\!\!\!\!-$}}
\newcommand{\commutesWith}{\sharp}
\newcommand{\notCommutesWith}{\not\sharp}
\newcommand{\rname}[1]{$\TirName{(#1)}$} % for inline inferrule names
\newcommand{\STO}{\ensuremath{<:}}  % ``subtype of''
\newcommand{\notSTO}{\ensuremath{\not<:}}  % ``subtype of''
\newcommand{\consistent}{\ensuremath{\approx}}

% auxiliary funtions for finding the dynamic effects for program executions.
\newcommand*{\dynamicInfinite}{\auxFunc{dynValue}}
\newcommand*{\dynamicEffects}{\auxFunc{dynE}}
\newcommand*{\dynamicEffectsOnce}{\auxFunc{dyn}}
\newcommand*{\dynamicEffectSet}{\auxFunc{dynESet}}
\newcommand*{\predecessorSiblings}{\auxFunc{preS}}
\newcommand*{\predSibles}{\auxFunc{pSib}}
%\newcommand*{\offspring}{\auxFunc{descendentsOf}}
%\newcommand*{\offspring}{\auxFunc{descendents}}
\newcommand*{\offspring}{\auxFunc{desc}}
\newcommand*{\offspringOrItself}{\auxFunc{descendOrSelf}} 
\newcommand*{\inQueueX}{\auxFunc{inQ}} 
\newcommand*{\inQueueY}{\auxFunc{inq}}
\newcommand*{\replaceQueue}{\auxFunc{replace}}
\newcommand*{\substituteSequence}{\auxFunc{subSeq}}
\newcommand*{\combineSequence}{\auxFunc{comSeq}}
\newcommand*{\mergeSequence}{\auxFunc{merSeq}}
\newcommand*{\isin}{\auxFunc{belongs}}
\newcommand*{\configuration}{c}

% Macros for operational semantics
\newcommand{\mc}[1]{\mbox{\rm \ensuremath{\text{\code{#1}}}}} % Arg set in code font in math
\newcommand{\loc}{\ensuremath{\mathord{\mathit{loc}}}}
\newcommand{\handler}[3]{\ensuremath{\langle#1,#2,#3\rangle}}
\newcommand{\ec}{\ensuremath{\mathbb{E}}}
%\newcommand{\ec}{\ensuremath{\mathop{\mathbb{E}}}}
%\newcommand{\ecpending}{\ensuremath{\mathop{\mathbb{E'}}}}
\newcommand{\ecpending}{\ensuremath{\mathop{\overline{\mathbb{E}}}}}
\newcommand{\hole}{\ensuremath{\mathord{\mathit{-}}}}
\newcommand{\reducesto}{\hookrightarrow}
\newcommand{\reducestostar}{\overset{*}{\reducesto}}
\newcommand{\dontcare}{\ensuremath{\mathord{\text{\textvisiblespace\hspace{0.10ex}}}}}
\newcommand{\Expression}{\ensuremath{{\cal E}}}
\newcommand{\Stack}{\mbox{\textit{Stack}}}
\newcommand{\Store}{\mbox{\textit{Store}}}
\newcommand{\ActiveList}{\mbox{\textit{ActiveList}}}
\newcommand{\Frame}{\mbox{\textit{Frame}}}
\newcommand{\FieldEnv}{\mbox{\textit{FieldEnv}}}
\newcommand{\ObjectRecord}{\mbox{\textit{ObjectRecord}}}
\newcommand{\lexframe}{\mbox{\textbf{\texttt{frame}}}}
\newcommand{\handlerframe}{\mbox{\textbf{\texttt{hframe}}}}
\newcommand{\Excep}{\mbox{\textit{Excep}}}

\newcommand*{\seq}[1]{\ensuremath{\left\langle {#1} \right\rangle}} % Arg is sequence contents
\newcommand{\config}{\seq}
\newcommand{\udot}{\mathbin{\sqcup \kern-0.53em \cdot \,}}

\newcommand{\eseq}{\hat{e}}

% Effect attributes
\newcommand{\ReadE}{\mbox{\texttt{\textbf{read}}~}}
%\newcommand{\WriteE}{\mbox{\texttt{\textbf{write}}~}}
\newcommand{\WriteE}{\mbox{\texttt{\textbf{write}}~}}
\newcommand{\CheckE}{\mbox{\texttt{\textbf{open}}}}
%\newcommand{\ForkE}{\mbox{\texttt{\textbf{fork}}}}
\newcommand{\ForkE}{\mbox{\texttt{\textbf{fork}}}}
\newcommand{\EnqueueE}{\mbox{\texttt{\textbf{bottom}}}}
%\newcommand{\BottomE}{\mbox{\texttt{\textbf{\bot}}}}
\newcommand{\RegisterE}{\mbox{\texttt{\textbf{exp}}}}
%\newcommand{\AnnounceE}{\mbox{\texttt{\textbf{frk}}~}}
\newcommand{\CreateE}{\mbox{\texttt{\textbf{create}}~}}
% Effect Auxiliary Functions
\newcommand*{\EffectsOf}{\auxFunc{effects}}
\newcommand{\ReadF}{\mbox{\texttt{\textbf{rd}}}}
\newcommand{\WriteF}{\mbox{\texttt{\textbf{wt}}}}
\newcommand{\ForkF}{\mbox{\texttt{\textbf{fk}}}}
\newcommand{\EnqueueF}{\mbox{\texttt{\textbf{eq}}}}
\newcommand{\BottomF}{\mbox{\texttt{\textbf{bt}}}}
\newcommand{\ConcretizedF}{\mbox{\texttt{\textbf{ct}}}}
\newcommand{\OtherF}{\mbox{\texttt{\textbf{el}}}}


\newcommand{\Class}{\mbox{\texttt{\textbf{class}}~}}
\newcommand{\Open}{\mbox{\texttt{\textbf{@open}}~}}
\newcommand{\Commute}{\mbox{\texttt{\textbf{@commute}}~}}
\newcommand{\tasks}{\mbox{\texttt{\textbf{tasks}}~}}
\newcommand{\fork}{\mbox{\texttt{\textbf{fork}}~}}
\newcommand{\foreach}{\mbox{\texttt{\textbf{forall}}~}}
\newcommand{\Decl}{\mbox{\texttt{\textbf{decl}}~}}
\newcommand{\RDecl}{\mbox{\texttt{\textbf{rdecl}}~}}
\newcommand{\Exp}{\mbox{\texttt{\textbf{exp}}~}}
\newcommand{\Prog}{\mbox{\texttt{\textbf{prog}}~}}
\newcommand{\Meth}{\mbox{\texttt{\textbf{meth}}~}}
\newcommand{\Type}{\mbox{\texttt{\textbf{type}}}}
\newcommand{\var}{\mbox{\textit{var}}}
\newcommand{\Nil}{\ensuremath{\bullet}}
\newcommand{\st}{\ensuremath{\textrm{s.t.}}}
\newcommand{\true}{\ensuremath{\mathit{true}}}
\newcommand{\false}{\ensuremath{\mathit{false}}}
\newcommand{\Land}{\ensuremath{\bigwedge}}

% New Panini features
\newcommand{\Announce}{\mbox{\texttt{\textbf{announce}}~}}
\newcommand{\Yield}{\mbox{\texttt{\textbf{yield}}~}}
%\newcommand{\Future}{\mbox{\texttt{\textbf{Future}}~}}

% names of the applications
\newcommand{\findbugs}{FindBugs}
\newcommand{\ga}{Genetic Algorithm}
\newcommand{\jasen}{jASEN}
\newcommand{\webcrawler}{WebSPHINX}
\newcommand{\refactoringcrawler}{RefactoringCrawler}

% Auxiliary functions for Panini
\newcommand*{\handlerSearch}{\auxFunc{hfind}}
\newcommand*{\handlerContexts}{\auxFunc{spawn}}
\newcommand*{\unroll}{\auxFunc{exec}}
\newcommand*{\buildContexts}{\auxFunc{buildconfs}}
%\newcommand*{\buildContext}{\auxFunc{buildconf}}
\newcommand*{\buildContext}{\auxFunc{build}}
\newcommand{\exclude}{\auxFunc{excl}}

\newcommand{\When}{\mbox{\texttt{\textbf{when}}}}
\newcommand{\Do}{\mbox{\texttt{\textbf{do}}}}
\newcommand{\Return}{\mbox{\texttt{\textbf{return}}}}
\newcommand{\Invoke}{\mbox{\texttt{\textbf{invoke}}}}
\newcommand{\Thunk}{\mbox{\texttt{\textbf{thunk}}~}}
\newcommand{\Register}{\mbox{\texttt{\textbf{register}}}}
\newcommand{\EventClosure}{\mbox{\texttt{\textbf{eClosure}}}}
\newcommand{\Boolean}{\mbox{\texttt{\textbf{boolean}}}}
\newcommand{\Int}{\mbox{\texttt{\textbf{int}}}}
\newcommand{\Void}{\mbox{\texttt{\textbf{void}}}}
\newcommand{\Nat}{\mbox{\texttt{\textbf{Nat}}}}

% auxiliary funtions for updating the event hierarchies
%\newcommand*{\updateGamma}{\auxFunc{updateHierarchy}}
\newcommand*{\updateGamma}{\auxFunc{updateHier}}
\newcommand*{\inGamma}{\auxFunc{registered}}
\newcommand*{\inDelta}{\auxFunc{inHierarchy}}
\newcommand*{\inZeta}{\auxFunc{inList}}
%\newcommand*{\updateEffect}{\auxFunc{updateEffect}}
\newcommand*{\collectBindings}{\auxFunc{colEvts}}
\newcommand*{\collectEvents}{\auxFunc{colEvt}}
\newcommand*{\putEvent}{\auxFunc{putEvent}}
\newcommand*{\putHierarchies}{\auxFunc{putHierarchies}}
\newcommand*{\putLevel}{\auxFunc{putLevel}}
\newcommand*{\effectsHierachy}{\auxFunc{effHier}}
\newcommand*{\effectsList}{\auxFunc{effList}}
\newcommand*{\effectsUnion}{\auxFunc{effUn}}
\newcommand*{\mergeRho}{\auxFunc{mergeRho}}
\newcommand*{\mergeEpsilon}{\auxFunc{mergeEff}}
\newcommand*{\effectEnlarge}{\auxFunc{effectEnlarge}}
\newcommand*{\insertLast}{\auxFunc{insert}}
\newcommand*{\compareLast}{\auxFunc{comp}}
\newcommand*{\build}{\auxFunc{build}}
\newcommand*{\isConcurrent}{\auxFunc{parallel}}
\newcommand*{\conflict}{\auxFunc{disjointMeth}}
\newcommand*{\disjoint}{\auxFunc{disj}}
\newcommand*{\interfere}{\auxFunc{nonConfl}}
\newcommand*{\deepCopy}{\auxFunc{copy}}
\newcommand*{\findMax}{\auxFunc{fresh}}
\newcommand*{\forkTask}{\auxFunc{buildconfs}}
\newcommand*{\intersect}{\auxFunc{intersect}}
\newcommand*{\inQueue}{\auxFunc{inQueue}}
\newcommand*{\copyEffect}{\auxFunc{cp}}
\newcommand*{\getTask}{\auxFunc{getTask}}
\newcommand*{\getFirstTask}{\auxFunc{getfirst}}

% Other stuff
\def\minimao#1{Mini\-MAO$_{#1}$\xspace}

% An environment for boxed figures
\usepackage{float}
\newenvironment{boxedfigure}
{
\floatstyle{boxed} 
\restylefloat{figure}
\begin{figure}[htb]
\em}
{
\end{figure}
\floatstyle{plain} 
\restylefloat{figure}
}

\newcommand*{\code}[1]{\texttt{#1}}

\definecolor{Brown}{cmyk}{0,0.81,1,0.60}
\definecolor{OliveGreen}{cmyk}{0.64,0,0.95,0.40}
\definecolor{CadetBlue}{cmyk}{0.62,0.57,0.23,0}
\definecolor{lightlightgray}{gray}{0.9}

\lstset{
language=Java,                            % Code langugage
basicstyle=\ttfamily,                     % Code font, Examples: \footnotesize, \ttfamily
keywordstyle=\color{OliveGreen}\bfseries, % Keywords font ('*' = uppercase)
commentstyle=\color{gray},                % Comments font
numbers=left,                             % Line nums position
numberstyle=\tiny,                        % Line-numbers fonts
stepnumber=1,                             % Step between two line-numbers
numbersep=5pt,                            % How far are line-numbers from code
backgroundcolor=\color{lightlightgray},   % Choose background color
frame=none,                               % A frame around the code
tabsize=2,                                % Default tab size
captionpos=b,                             % Caption-position = bottom
breaklines=true,                          % Automatic line breaking?
breakatwhitespace=false,                  % Automatic breaks only at whitespace?
showspaces=false,                         % Dont make spaces visible
showtabs=false,                           % Dont make tabls visible
%columns=flexible,                        % Column format
morekeywords={%                           % Language specific keywords
  cast,do,under,loc,yield,commit,forAll,doAll,ref,let,$\lambda$,in}
}

% % Settings for the listings package
% \lstset{%
% language=[AspectJ]Java,%
% basicstyle=\rmfamily,%\sffamily,% \ttfamily,%
% commentstyle=\ttfamily,%
% numbers=left,%
% numberstyle=\tiny,%
% numbersep=2pt,%
% numberblanklines=false,%
% morekeywords={%
% cast,do,under,loc,yield,commit,forAll,doAll,ref,let,$\lambda$,in}}

% could use \relsize{-2} instead of \scriptsize below
\newcommand{\FIGCODEFONT}{\relsize{-1}\ttfamily}
\newcommand{\FIGCODELIBFONT}{\relsize{-6}\ttfamily}

% cross referencing
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\fignref}[1]{Figure~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\secnref}[1]{Section~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\theref}[1]{Theorem~\ref{#1}}
\newcommand{\lineref}[1]{line~\ref{#1}}
\newcommand{\linesref}[2]{lines~\ref{#1}-\ref{#2}}
\newcommand{\linerefNum}[1]{\ref{#1}}
\newcommand{\footnoteref}[1]{$^{\ref{#1}}$}

% {theorems}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}
%Some helpful notation
\newcommand{\PROOF}{{\em Proof:\/}~~}

\newcommand{\etal}{~\textit{et al.}}

% used in def-use project only
\newcommand{\ClosestDecl}{Closest Declaration Analysis}
\newcommand{\CloserDecl}{closer declaration analysis}
\newcommand{\CloserDeclarationTool}{CloDecl}
\newcommand{\SomeProperty}{P}
\newcommand{\DefUse}{Def-Use Idiom}
\newcommand{\SemiPurity}{Observational Purity}
\newcommand{\DefF}{\mbox{\texttt{\textbf{def}}~}}
\newcommand{\UseF}{\mbox{\texttt{\textbf{use}}~}}
% data race free definition
\newcommand{\DefUseStaticF}{\auxFunc{DefUseStatic}}
\newcommand{\DefUseInstanceF}{\auxFunc{DefUseInstance}}
% Auxiliary functions for CloestDecl
\newcommand{\predecessor}{\auxFunc{pred}}
\newcommand{\AnalysisSets}{Read-Write Sets}
\newcommand{\MethodCall}{\auxFunc{Call}}

%\newcommand{\PROOFSKETCH}{{\em Proof Sketch:\/}~~}
\newcommand{\PROOFSKETCH}{{\em Proof:\/}~~}
\newcommand{\QED}{\rule{0.4em}{0.65em}}

%\definecolor{lightest-gray}{rgb}{0.95,0.95,0.5} % for talks
\definecolor{lightest-gray}{gray}{0.97}
%\definecolor{lighter-gray}{rgb}{0.7,0.98,0.7} % for talks
\definecolor{lighter-gray}{gray}{0.93}
%\definecolor{light-gray}{rgb}{0.5,0.98,0.98} % for talks
\definecolor{light-gray}{gray}{0.89}
%\definecolor{dark-gray}{rgb}{0.95,0.7,0.95} % for talks
\definecolor{dark-gray}{gray}{0.85}
%\definecolor{darker-gray}{rgb}{1,0.65,0.65} % for talks
\definecolor{darker-gray}{gray}{0.81}

%\newcommand\para[1]{\vspace{0.0em}\paragraph{{\bf #1.}\ }}
\newcommand\para[1]{\paragraph{#1}}

% formatting of initial section quotations
\newcommand{\QUOTATION}[1]{\begin{flushright}\emph{#1}\end{flushright}}

% \newtheorem{theorem}{{\bf Theorem}}[section]
% \newenvironment{definition}[1][Definition]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% 
% \newenvironment{lemma}[1][Lemma]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% 
% \newenvironment{example}[1][Example]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% 
% \newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

% \newcommand{\qed}{\nobreak \ifvmode \relax \else
%       \ifdim\lastskip<1.5em \hskip-\lastskip
%       \hskip1.5em plus0em minus0.5em \fi \nobreak
%       \vrule height0.75em width0.5em depth0.25em\fi}

% Allow figures to take up the entire page
\renewcommand\floatpagefraction{.99}
\renewcommand\topfraction{.99}
\renewcommand\bottomfraction{.90}
\renewcommand\textfraction{.01}

% \renewcommand{\topfraction}{0.90}
% \renewcommand{\textfraction}{0.05}
% \renewcommand{\floatpagefraction}{0.85}

==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}

